A Tree Clock Data Structure for Causal Orderings in Concurrent Executions

Dynamic techniques are a scalable and effective way to analyze concurrent programs. Instead of analyzing all behaviors of a program, these techniques detect errors by focusing on a single program execution. Often a crucial step in these techniques is to define a causal ordering between events in the execution, which is then computed using vector clocks, a simple data structure that stores logical times of threads. The two basic operations of vector clocks, namely join and copy, require $\Theta(k)$ time, where $k$ is the number of threads. Thus they are a computational bottleneck when $k$ is large. In this work, we introduce tree clocks, a new data structure that replaces vector clocks for computing causal orderings in program executions. Joining and copying tree clocks takes time that is roughly proportional to the number of entries being modified, and hence the two operations do not suffer the a-priori $\Theta(k)$ cost per application. We show that when used to compute the classic happens-before (HB) partial order, tree clocks are optimal, in the sense that no other data structure can lead to smaller asymptotic running time. Moreover, we demonstrate that tree clocks can be used to compute other partial orders, such as schedulable-happens-before (SHB) and the standard Mazurkiewicz (MAZ) partial order, and thus are a versatile data structure. Our experiments show that just by replacing vector clocks with tree clocks, the computation becomes from $2.02 \times$ faster (MAZ) to $2.66 \times$ (SHB) and $2.97 \times$ (HB) on average per benchmark. These results illustrate that tree clocks have the potential to become a standard data structure with wide applications in concurrent analyses.

==> algorithms/algo_clock_tree2.tex <==
\small
\begin{algorithm*}[!h]
% \BlankLine
\begin{multicols}{2}
%\MyFunction{\FunctionCTJoin{$\TreeClock'$}}{
Let $z'\gets \TreeClock'.\GTree.\Root$\\
\uIf{$z'.\clock \leq \FunctionCTGet(z'.\tid)$}{
\Return 
}
Let $\Stack\gets$ an empty stack\\
\tcp{Handle the root}
Let $v'\gets z'.\First$\\
\While{$v'\neq \bot$}{
\eIf{$\FunctionCTGet(v'.\tid) < v'.\clock$}{
Push $v'$ in $\Stack$
}
{
\uIf{$v'.\pclock \leq \FunctionCTGet(z'.\tid)$}{
\Break
}
}
Assign $v'\gets v'.\Right$
}
\tcp{Detach $z'.\tid$ from $\GTree$}
Let $u\gets \ThreadMap(z'.\tid)$\\
\uIf{$u.\Right\neq \bot$}{
Assign $u.\Right.\Left\gets u.\Left$
}
\eIf{$u.\Left\neq \bot$}{
Assign $u.\Left.\Right\gets u.\Right$\\
}
{
Assign $u.\Parent.\First\gets u.\Right$
}
\tcp{Update the clock of $u$}
Assign $u.\clock\gets z'.\clock$\\
\tcp{Place the updated subtree under the root of $\GTree$}
Let $z\gets \GTree.\Root$\\
Assign $u.\pclock\gets z.\clock$\\
\uIf{$z.\First \neq \bot$}{
Assign $z.\First.\Left\gets u$
}
Assign $u.\Left\gets \bot$\\
Assign $u.\Right\gets z.\First$\\
Assign $u.\Parent\gets z$\\
Assign $z.\First\gets u$\\
\tcp{Handle the rest}
\While{$\Stack$ is not empty}{
Let $u'\gets$ pop $\Stack$\\
\tcp{Expand to children of $u'$}
Let $v'\gets u'.\First$\\
\While{$v'\neq \bot$}{
%\ForEach{$v'$ in $\ChildrenQ(u')$}{
\eIf{$\FunctionCTGet(v'.\tid) < v'.\clock$}{
Push $v'$ in $\Stack$
}
{
\uIf{$v'.\pclock \leq \FunctionCTGet(u'.\tid)$}{
\Break
}
}
Assign $v'\gets v'.\Right$
}
\tcp{Detach $u'.\tid$ from $\GTree$}
Let $u\gets \ThreadMap(u'.\tid)$\\
\uIf{$u.\Right\neq \bot$}{
Assign $u.\Right.\Left\gets u.\Left$
}
\eIf{$u.\Left\neq \bot$}{
Assign $u.\Left.\Right\gets u.\Right$\\
}
{
Assign $u.\Parent.\First\gets u.\Right$
}
\tcp{Update the clock of $u$}
Assign $u.\clock\gets u'.\clock$\\
Assign $u.\pclock\gets u'.\pclock$\\
\tcp{Attach back}
Let $y\gets \ThreadMap(u'.\Parent.\tid)$\\
\uIf{$y.\First \neq \bot$}{
Assign $y.\First.\Left\gets u$
}
Assign $u.\Left\gets \bot$\\
Assign $u.\Right\gets y.\First$\\
Assign $u.\Parent\gets y$\\
Assign $y.\First\gets u$\\
}
%}
\end{multicols}
\normalsize
\caption{
Join without function calls.
}
\label{algo:join}
\end{algorithm*}







\small
\begin{algorithm*}[!h]
% \BlankLine
\begin{multicols}{2}
\BlankLine
%\tcp*[f]{}
Let $z'\gets\TreeClock'.\GTree.\Root$\\
Let $z\gets\GTree.\Root$\\ 
Let $\Stack\gets$ an empty stack\\
\tcp{Handle the root}
Let $v'\gets z'.\First$\\
\While{$v'\neq \bot$}{
%\ForEach{$v'$ in $\ChildrenQ(z')$}{
\eIf{$\FunctionCTGet(v'.\tid) < v'.\clock$}{
Push $v'$ in $\Stack$
}
{
\uIf{$v'\tid==z.\tid$}{
Push $v'$ in $\Stack$
}
\uIf{$v'.\pclock \leq \FunctionCTGet(z'.\tid)$}{
\Break
}
}
Assign $v'\gets v'.\Right$
}
\tcp{Detach $z'.\tid$ from $\GTree$}
Let $u\gets \ThreadMap(z'.\tid)$\\
\uIf{$u.\Right\neq \bot$}{
Assign $u.\Right.\Left\gets u.\Left$
}
\eIf{$u.\Left\neq \bot$}{
Assign $u.\Left.\Right\gets u.\Right$\\
}
{
Assign $u.\Parent.\First\gets u.\Right$
}
\tcp{Update the clock of $u$}
Assign $u.\clock\gets z'.\clock$\\
\tcp{Make $u$ the root}
Assign $u.\Left\gets \bot$\\
Assign $\GTree.\Root\gets u$\\
\tcp{Handle the rest}
\While{$\Stack$ is not empty}{
Let $u'\gets$ pop $\Stack$\\
\tcp{Expand to children of $u'$}
Let $v'\gets u'.\First$\\
\While{$v'\neq \bot$}{
\eIf{$\FunctionCTGet(v'.\tid) < v'.\clock$}{
Push $v'$ in $\Stack$
}
{
\uIf{$v'\tid==z.\tid$}{
Push $v'$ in $\Stack$
}
\uIf{$v'.\pclock \leq \FunctionCTGet(u'.\tid)$}{
\Break
}
}
Assign $v'\gets v'.\Right$
}
\tcp{Detach $u'.\tid$ from $\GTree$}
Let $u\gets \ThreadMap(u'.\tid)$\\
\uIf{$u.\Right\neq \bot$}{
Assign $u.\Right.\Left\gets u.\Left$
}
\eIf{$u.\Left\neq \bot$}{
Assign $u.\Left.\Right\gets u.\Right$\\
}
{
Assign $u.\Parent.\First\gets u.\Right$
}
\tcp{Update the clock of $u$}
Assign $u.\clock\gets u'.\clock$\\
Assign $u.\pclock\gets u'.\pclock$\\
\tcp{Attach back}
Let $y\gets \ThreadMap(u'.\Parent.\tid)$\\
\uIf{$y.\First \neq \bot$}{
Assign $y.\First.\Left\gets u$
}
Assign $u.\Left\gets \bot$\\
Assign $u.\Right\gets y.\First$\\
Assign $u.\Parent\gets y$\\
Assign $y.\First\gets u$\\
}
\end{multicols}
\normalsize
\caption{
MonotoneCopy without function calls.
}
\label{algo:monotonecopy}
\end{algorithm*}

==> algorithms/algo_dc.tex <==
\small
\begin{algorithm}
% \BlankLine
\BlankLine
%\tcp*[f]{}
\MyProcedure{\ProcAcquire{$\Thread$, $\ell$}}{
\lForEach{$\Thread'\neq \Thread$}{
$\AcquireQueue_{\Thread', \ell}(\Thread).\Enqueue(\CTC_{\Thread})$\label{line:dc_joinacquire}
}
}
\BlankLine
\BlankLine
\MyProcedure{\ProcRelease{$\Thread$, $\ell$}}{
\ForEach{$\Thread'\neq \Thread$}{
\While{$\AcquireQueue_{\Thread,\ell}(\Thread').\Front().\FunctionCTLessThan(\CTC_{\Thread})$}{
$\AcquireQueue_{\Thread, \ell}(\Thread').\Dequeue()$\\
$\CTC_{\Thread}.\FunctionCTJoin(\ReleaseQueue_{\Thread, \ell}(\Thread').\Dequeue())$
}
}
\lForEach{$x\in \ReadsSet_{\ell}$}{
$\CTL_{\ell, x}^{\Read}.\FunctionCTMonotoneCopy(\CTC_{\Thread})$\label{line:dc_copyread}
}
\lForEach{$x\in \WritesSet_{\ell}$}{
$\CTL_{\ell, x}^{\Write}.\FunctionCTMonotoneCopy(\CTC_{\Thread})$\label{line:dc_copywrite}
}
$\ReadsSet_{\ell}\gets \emptyset$~;
$\WritesSet_{\ell}\gets \emptyset$\\
\lForEach{$\Thread'\neq \Thread$}{
$\ReleaseQueue_{\ell, \Thread'}(\Thread).\Enqueue(\CTC_{\Thread})$
}
}
\BlankLine
\BlankLine
\MyProcedure{\ProcRead{$\Thread$, $x$}}{
\ForEach{$\ell\in \HeldLocks(\Thread)$}{
$\CTC_{\Thread}.\FunctionCTJoin(\CTL_{\ell, x}^{\Write})$~;
$\ReadsSet_{\ell}\gets \ReadsSet_{\ell} \cup \{ x \}$\label{line:dc_readjoin}
}
}
\BlankLine
\BlankLine
\MyProcedure{\ProcWrite{$\Thread$, $x$}}{
\ForEach{$\ell\in \HeldLocks(\Thread)$}{
$\CTC_{\Thread}.\FunctionCTJoin(\CTL_{\ell, x}^{\Write})$~;
$\CTC_{\Thread}.\FunctionCTJoin(\CTL_{\ell, x}^{\Read})$~;
$\WritesSet_{\ell}\gets \WritesSet_{\ell} \cup \{ x \}$\label{line:dc_writejoin}
}
}
\normalsize
\caption{
$\DC$ with tree clocks.
}
\label{algo:dc}
\end{algorithm}
\normalsize

==> algorithms/algo_fasthb.tex <==
\small
\begin{algorithm}
% \BlankLine
\BlankLine
%\tcp*[f]{}
\MyProcedure{\ProcInitialize{}}{

\ForEach{thread $\Thread$}{
$\CTC_{\Thread}.\FunctionCTInitialize()$
}
\ForEach{lock $\ell$}{
Declare a tree clock $\CTL_{\ell}$
}

\ForEach{variable $x$}{
Let $\EpochWrite_x\gets \bot$ \tcp*{$(\tid, \clock)$ of last write}
Let $\VCR_{x}\gets \bot$ \tcp*{Vector clock of last reads}
Let $\EpochReads_x\gets \emptyset$ \tcp*{Threads of last reads}
}
}
\BlankLine
\BlankLine
\MyProcedure{\ProcAcquire{$\Thread$, $\ell$}}{
$\CTC_{\Thread}.\FunctionCTJoin(\CTL_{\ell})$
}
\BlankLine
\BlankLine
\MyProcedure{\ProcRelease{$\Thread$, $\ell$}}{
$\CTL_{\ell}.\FunctionCTMonotoneCopy(\CTC_{\Thread})$
}
\BlankLine
\BlankLine
\MyProcedure{\ProcRead{$\Thread$, $x$}}{
\uIf{$\CTC_{\Thread}.\FunctionCTGet(\EpochWrite_x.\tid) < \EpochWrite_x.\clock$ }{
Report read-write race on $x$\\
}
Assign $\VCR_{x}[\Thread]\gets \CTC_{\Thread}.\FunctionCTGet(\Thread)$\\
Assign $\EpochReads_x \gets \EpochReads_x(\Thread) \cup \{ \Thread \}$\\
}
\BlankLine
\BlankLine
\MyProcedure{\ProcWrite{$\Thread$, $x$}}{
\uIf{$\CTC_{\Thread}.\FunctionCTGet(\EpochWrite_x.\tid) < \EpochWrite_x.\clock$ }{
Report write-write race on $x$\\
}
\ForEach{$\Thread'\in \EpochReads_x$}{
\uIf{$\CTC_{\Thread}.\FunctionCTGet(\EpochWrite_x.\tid) < \VCR_{x}[\Thread']$ }{
Report write-read race on $x$\\
}
}
Assign $\EpochWrite_x\gets (\Thread, \CTC_{\Thread}.\FunctionCTGet(\Thread))$\\
Assign $\EpochReads_x\gets \emptyset$\\
}
\normalsize
\caption{
$\FastHB$
}
\label{algo:fasthb}
\end{algorithm}
\normalsize

==> algorithms/algo_sdp.tex <==
\small
\begin{algorithm}
% \BlankLine
\BlankLine
%\tcp*[f]{}
\MyProcedure{\ProcAcquire{$\Thread$, $\ell$}}{
$\CTH_{\Thread}.\FunctionCTJoin(\CTH_{\ell})$~;
$\CTP_{\Thread}.\FunctionCTSubRootJoin(\CTP_{\ell})$\\
\lForEach{$\Thread'\neq \Thread$}{
$\AcquireQueue_{\ell}(\Thread').\Enqueue( (\Thread, \LocalTime{}{\Event}))$
}
}
\BlankLine
\BlankLine
\MyProcedure{\ProcRelease{$\Thread$, $\ell$}}{
%\While{$\AcquireQueue_{\ell}(\Thread).\Front().\FunctionCTLessThan(\CTH_{\Thread})$}{
\While{\RoutineTestDeque($\AcquireQueue_{\ell}(\Thread).\Front(), \CTP_{\Thread}, \Thread$)}{
$\AcquireQueue_{\ell}(\Thread).\Dequeue()$~;
$\CTP_{\Thread}.\FunctionCTJoin(\ReleaseQueue_{\ell}(\Thread).\Dequeue())$\\
}
\lForEach{$x\in \ReadsSet_{\ell}$}{
$\CTL_{\ell, x}^{\Read}.\FunctionCTMonotoneCopy(\CTH_{\Thread})$\label{line:sdp_copyread}
}
\lForEach{$x\in \WritesSet_{\ell}$}{
$\CTL_{\ell, x}^{\Write}.\FunctionCTMonotoneCopy(\CTH_{\Thread})$\label{line:sdp_copywrite}
}
$\ReadsSet_{\ell}\gets \emptyset$~;
$\WritesSet_{\ell}\gets \emptyset$\\
$\CTH_{\ell}.\FunctionCTMonotoneCopy(\CTH_{\Thread})$~;
$\CTP_{\ell}.\FunctionCTMonotoneCopy(\CTP_{\Thread})$\\
\lForEach{$\Thread'\neq \Thread$}{
$\ReleaseQueue_{\ell}(\Thread').\Enqueue(\CTH_{\ell})$
}
}
\BlankLine
\BlankLine
\MyProcedure{\ProcRead{$\Thread$, $x$}}{
\ForEach{$\ell\in \HeldLocks(\Thread)$}{
$\CTP_{\Thread}.\FunctionCTSubRootJoin(\CTB_{\Thread, x}^{\Write})$~;
$\CTP_{\Thread}.\FunctionCTSubRootJoin(\CTL_{\ell, x}^{\Write})$~;
$\ReadsSet_{\ell}\gets \ReadsSet_{\ell} \cup \{ x \}$\label{line:sdp_readjoin}
}
}
\BlankLine
\BlankLine
\MyProcedure{\ProcWrite{$\Thread$, $x$}}{
\ForEach{$\ell\in \HeldLocks(\Thread)$}{
$\CTB_{\Thread, x}.\FunctionCTSubRootJoin(\CTL_{\ell, x}^{\Write})$~;\label{line:sdp_writesubjoin1}
$\CTP_{\Thread}.\FunctionCTSubRootJoin(\CTL_{\ell, x}^{\Read})$~;\label{line:sdp_writesubjoin2}
$\WritesSet_{\ell}\gets \WritesSet_{\ell} \cup \{ x \}$\label{line:sdp_writejoin}
}
}
\BlankLine
\BlankLine
\MyRoutine{\RoutineTestDeque{$(\tid, \clock), \CTP, \Thread$}}{
\eIf{$\tid==\Thread$}{
\Return{$\True$}
}{
\Return{ $\clock \leq \CTP.\FunctionCTGet(\tid)$ }
}
}
\normalsize
\caption{
$\SDP$ with tree clocks.
}
\label{algo:sdp}
\end{algorithm}
\normalsize

==> algorithms/algo_wcp.tex <==
\small
\begin{algorithm}
% \BlankLine
\BlankLine
%\tcp*[f]{}
\MyProcedure{\ProcAcquire{$\Thread$, $\ell$}}{
$\CTH_{\Thread}.\FunctionCTJoin(\CTH_{\ell})$~;
$\CTP_{\Thread}.\FunctionCTSubRootJoin(\CTP_{\ell})$\\
\lForEach{$\Thread'\neq \Thread$}{
$\AcquireQueue_{\ell}(\Thread').\Enqueue( (\Thread, \LocalTime{}{\Event}))$
}
}
\BlankLine
\BlankLine
\MyProcedure{\ProcRelease{$\Thread$, $\ell$}}{
%\While{$\AcquireQueue_{\ell}(\Thread).\Front().\FunctionCTLessThan(\CTH_{\Thread})$}{
\While{\RoutineTestDeque($\AcquireQueue_{\ell}(\Thread).\Front(), \CTP_{\Thread}, \Thread$)}{
$\AcquireQueue_{\ell}(\Thread).\Dequeue()$~;
$\CTP_{\Thread}.\FunctionCTJoin(\ReleaseQueue_{\ell}(\Thread).\Dequeue())$\\
}
\lForEach{$x\in \ReadsSet_{\ell}$}{
$\CTL_{\ell, x}^{\Read}.\FunctionCTMonotoneCopy(\CTH_{\Thread})$\label{line:wcp_copyread}
}
\lForEach{$x\in \WritesSet_{\ell}$}{
$\CTL_{\ell, x}^{\Write}.\FunctionCTMonotoneCopy(\CTH_{\Thread})$\label{line:wcp_copywrite}
}
$\ReadsSet_{\ell}\gets \emptyset$~;
$\WritesSet_{\ell}\gets \emptyset$\\
$\CTH_{\ell}.\FunctionCTMonotoneCopy(\CTH_{\Thread})$~;
$\CTP_{\ell}.\FunctionCTMonotoneCopy(\CTP_{\Thread})$\\
\lForEach{$\Thread'\neq \Thread$}{
$\ReleaseQueue_{\ell}(\Thread').\Enqueue(\CTH_{\ell})$
}
}
\BlankLine
\BlankLine
\MyProcedure{\ProcRead{$\Thread$, $x$}}{
\ForEach{$\ell\in \HeldLocks(\Thread)$}{
$\CTP_{\Thread}.\FunctionCTSubRootJoin(\CTL_{\ell, x}^{\Write})$~;\label{line:wcp_readsubjoin}
$\ReadsSet_{\ell}\gets \ReadsSet_{\ell} \cup \{ x \}$\label{line:wcp_readjoin}
}
}
\BlankLine
\BlankLine
\MyProcedure{\ProcWrite{$\Thread$, $x$}}{
\ForEach{$\ell\in \HeldLocks(\Thread)$}{
$\CTP_{\Thread}.\FunctionCTSubRootJoin(\CTL_{\ell, x}^{\Write})$~;\label{line:wcp_writesubjoin1}
$\CTP_{\Thread}.\FunctionCTSubRootJoin(\CTL_{\ell, x}^{\Read})$~;\label{line:wcp_writesubjoin2}
$\WritesSet_{\ell}\gets \WritesSet_{\ell} \cup \{ x \}$\label{line:wcp_writejoin}
}
}
\BlankLine
\BlankLine
\MyRoutine{\RoutineTestDeque{$(\tid, \clock), \CTP, \Thread$}}{
\eIf{$\tid==\Thread$}{
\Return{$\True$}
}{
\Return{ $\clock \leq \CTP.\FunctionCTGet(\tid)$ }
}
}
\normalsize
\caption{
$\WCP$ with tree clocks.
}
\label{algo:wcp}
\end{algorithm}
\normalsize

==> app_exp.tex <==
\section{Experimental Details of VT-Work}

\input{tables/counters}

In this section we present more statistics on the number of operations that tree clocks and vector clocks perform on our dataset.
For each benchmark we have computed
\begin{compactenum}
\item The vt-work that was needed for that benchmark, i.e., the total number of vector-time entries that were updated during the execution of the benchmark under the $\HB$ and $\SHB$ partial order.
This corresponds to the dark-gray areas of our figures (e.g., \cref{fig:ctjoin}).
\item The tree-clock work that was done for that benchmark, i.e., the total number of nodes of tree clocks that were accessed by the tree-clock join and copy operations.
This corresponds to the light-gray areas of our figures (e.g., \cref{fig:ctjoin}).
\item The vector-clock work that was done for that benchmark, i.e., the total number of entries of vector clocks that were accessed by the vector-clock join and copy operations.
\end{compactenum}
 \cref{tab:counters} shows the obtained results.



==> app_race_predictors.tex <==
\section{Tree Clocks in More Race Prediction}\label{sec:app_race_predictors}

In this section we show how tree clocks can replace vector clocks for computing the $\DC$~\cite{Roemer18} and $\SDP$~\cite{Genc19} partial orders.

\input{dc}
\input{sdp}

==> atomicity.tex <==
\subsection{Tree Clocks in Atomicity Checking}\label{subsec:atomicity}

==> clocktrees.tex <==
\section{Race Detection with Clock Trees}\label{sec:clock_trees}

In this section we introduce clock trees, a new data structure for representing logical times in concurrent and distributed programs.
We first illustrate the intuition behind clock trees, and then present the formal details.

\input{intuition}

\input{clocktrees_details}

\input{optimality}


==> dc.tex <==
\subsection{Doesn't Commute}\label{subsec:dc}

\Paragraph{The $\DC$ partial order.}
Doesn't-commute is a partial order introduced in~\cite{Roemer18}.
It is an unsound weakening of $\WCP$, which means that it can report more races, but also make unsound reports.
Nevertheless, $\DC$ races are candidates of actual races, and are processed by a second, more heavyweight but sound phase.
$\DC$ races that do not pass this phase are vindicated, whereas the ones that pass are sound races.

\Paragraph{$\DC$ with tree clocks.}
\cref{algo:dc} shows $\DC$ using tree clocks.
It is a direct adaptation of the $\DC$ algorithm based on vector clocks~\cite{Roemer18}.
The only observation required is that the copies in \cref{line:dc_copyread,line:dc_copywrite} occurring when the algorithm processes a lock-release event $\Release$ are indeed monotone.
This monotonicity holds due to the corresponding joins in \cref{line:dc_readjoin} and \cref{line:dc_writejoin} 
that occur while the algorithm processes the critical section of $\Release$.


\input{algorithms/algo_dc}

==> distributed.tex <==
\section{Tree Clocks in Distributed Systems}\label{sec:tc_distributed}





==> experiments_old.tex <==
%!TEX root=main.tex

\section{Experiments}\label{sec:experiments}

In this section we report on an implementation and experimental evaluation of the tree clock data structure.
The primary goal of these experiments is to evaluate the practical advantage of tree clocks over the vector clocks for keeping track of logical times in a concurrent program.

\Paragraph{Implementation.}
Our implementation is in Java and closely follows \cref{algo:clock_tree}.
For efficiency reasons, recursive routines have been made iterative.
The thread map $\ThreadMap$ is implemented as a list with random access,
while the $\ChildrenQ(u)$ data structure for storing the children of node $u$ is implemented as a doubly linked list.
We also implemented \djitp style optimizations~\cite{Pozniansky03} for both tree and vector clocks.

\Paragraph{Benchmarks.}
Our benchmark set consists of standard benchmarks found in the recent literature. mostly in the context of race detection~\cite{Huang14,Kini17,Mathur18,Roemer18,Pavlogiannis2020,Mathur21}.
It contains several concurrent programs taken from standard benchmark 
suites --- IBM Contest benchmark suite~\cite{Farchi03}, Java Grande suite~\cite{Smith01},
DaCapo~\cite{Blackburn06}, and
SIR~\cite{doESE05}.
% \begin{compactenum}
% \item the IBM Contest benchmark suite~\cite{Farchi03},
% \item the Java Grande forum benchmark suite~\cite{Smith01},
% \item the DaCapo benchmark suite~\cite{Blackburn06}, and
% \item the Software Infrastructure Repository~\cite{doESE05}
% \end{compactenum}
% For each benchmark, we used the tool RV-Predict~\cite{rvpredict} to instrument it and monitor its execution, which created a single trace per program.
% The same trace was used for evaluating all algorithms.
In order to fairly compare the performance of vector clocks
and tree clocks, we logged the execution traces of each benchmark program 
using RV-Predict~\cite{rvpredict} and analyze both VC-based and TC-based algorithms on the same trace.

\Paragraph{Setup.}
Our experimental setup consists of two implementations for each of the $\HB$ and $\SHB$ algorithms, one using vector clocks and the other using tree clocks to represent vector times (\cref{algo:hb} and \cref{algo:shb}).
Each algorithm was given as input a trace produced from the above benchmarks, and we measured the running time to construct the respective partial order.
We do not include small benchmarks where this time is below 10ms,
as these cases are very simple to handle using vector clocks and 
the tree clock data structure is not likely to offer any advantage.
As our focus is on the impact of the vector-time data structure on timestamping, we did not perform any further analysis after constructing partial order (e.g., detecting races).
Although these partial orders are useful for various analyses,
we remark that any analysis component will be identical under vector clocks and tree clocks, and thus does not contribute to the comparison of the two data structures.


\input{tables/tab_times}

\begin{figure*}[t!]
\includegraphics[scale=0.7]{figures/vt_workHB}
\caption{Comparing number of operations (vt-work) performed using vector clocks and tree-clocks in $\HB$ (y-axis is log-scale).}
\label{fig:vtwork}
\end{figure*}

\Paragraph{Running times.}
The running times for vector clocks and tree clocks are shown in \cref{tab:times}.
We see that $\SHB$ requires significantly more time to construct than $\HB$, for  both vector clocks and tree clocks.
This is expected, as $\HB$ only orders synchronization events (i.e., release/acquire events) 
across threads, while $\SHB$ also orders memory access events  events.

We observe that tree clocks incur a significant speedup over vector clocks for both partial orders in most benchmarks.
In the case of $\HB$, the whole benchmark set is processed approximately $5.5$ times faster using tree clocks, while for $\SHB$ the speedup is $2.24$ times faster.
The speedup for $\SHB$ is less than $\HB$.
This is expected because $\SHB$ uses as many vector/tree clocks as there are variables.
However, for some of these variables, the corresponding vector/tree clock is only used in a few join and copy operations.
As the tree clock is a more heavy data structure, the number of these operations is not large enough to balance the initialization overhead of tree clocks.
Nevertheless, overall tree clocks deliver a generous speedup to both $\HB$ and $\SHB$.

To get a better aggregate representation of the advantage of tree clocks, we have also computed the geometric mean of the ratios of vector-clock times over tree-clock times, averaged over all benchmarks.
For $\HB$, the speedup is $\operatorname{GMean}_{\HB}=2$, while for $\SHB$ the speedup is  $\operatorname{GMean}_{\SHB}=1.75$.
These numbers show that just by replacing vector clocks with tree clocks, the running time reduces on average to $50\%$ for $\HB$ and to $57\%$ for $\SHB$, regardless of the total running time of the benchmark.
These are significant reductions, especially coming from using a new data structure without any attempt to optimize other aspects such as
the algorithm that constructs the respective partial order.

\Paragraph{Deep and monotone copies in $\SHB$.}
Recall that in $\SHB$ with tree clocks, the processing  of a write event leads to a $\FunctionCTCopyCheckMonotone$ operation,
which might resolve to a deep copy between the tree clocks instead of a monotone one (\cref{algo:shb}).
If the number of deep copies is large, the advantage of tree clocks is lost as the operation touches the whole data structure.
Here we have evaluated our expectation that the frequency of deep copies is negligible compared to monotone copies.
Indeed, we have seen that in all benchmarks, the number of deep copies is many orders of magnitude smaller than the number of monotone copies.
For a few representative numbers,  in the case zxing, $\FunctionCTCopyCheckMonotone$ resolved 137M times to a monotone copy and only 43 times to a deep copy.
In the case of hsqldb, the corresponding numbers are 2.3M and 25.
Analogous observations hold for all other benchmarks. 


\Paragraph{Comparison with vt-work.}
We also investigate the total number of entries updated using each of the data structures.
Recall that the metric $\VTWork(\Trace)$ (\cref{sec:race_detection})
measures the minimum amount of updates
that any implementation of the vector time must perform
when computing a partial order.
We can likewise define the metrics $\TCWork(\Trace)$ and
$\VCWork(\Trace)$ corresponding to the number of entries updated
when processing each event when using respectively the data structures
tree clocks and vector clocks.
These metrics are visualized in \cref{fig:vtwork} for our benchmark suite
and accurately explain the performance improvement of tree clocks
over vector clocks (\cref{tab:times}).
The figure shows that the $\VCWork(\Trace)/ \VTWork(\Trace)$ ratio is often considerably large.
In contrast, the ratio $\TCWork(\Trace)/ \VTWork(\Trace)$ is typically significantly smaller.
The differences in running times between vector and tree clocks are a
direct reflection of the discrepancies between $\TCWork(\cdot)$ and $\VCWork(\cdot)$.
In fact, the benchmarks which have the highest ratios $\TCWork(\Trace)/\VCWork(\Trace)$ 
also show a corresponding high speed-up
(cassandra, tradebeans, hsqldb and raxextended).
Next, we remark $\TCWork(\Trace)$ is 
always no more than a constant factor larger than $\VTWork(\Trace)$;
our proof of \cref{thm:vtoptimality} 
implies that $\TCWork(\Trace)\leq 3\cdot  \VTWork(\Trace)$.
The ratios in \cref{fig:vtwork} confirm this theoretical bound. 
Interestingly, for the benchmark bufwriter, we have $\TCWork(\Trace)\simeq 2.99\cdot  \VTWork(\Trace)$,
i.e., this benchmark pushes tree clocks to their worst performance relative to vt-work.




 


==> extended-abstract/key_insights.tex <==
\section{Key Insights}
\label{sec:key-insights}


\begin{itemize}
\item What are the one or two key new insights in this paper?
\item How does it advance the state of the art?
\item What makes it more effective than past approaches?
\end{itemize}


\vspace{2cm}


The key insight that this work is based on is that vector clock join and copy operations most of the time perform unnecessary updates.
For example, when thread $\Thread_1$ receives a message from $\Thread_2$, 
the whole vector clock of $\Thread_2$ is processed in order to update the view of $\Thread_1$ about all other threads in the system that $\Thread_2$ knows about.
However, if $\Thread_1$ knows of a later time for some thread $\Thread_3$ than $\Thread_2$ does, we ideally would like to \emph{a-priori} avoid checking $\Thread_3$ in the vector clock of $\Thread_2$.
Unfortunately, the flat structure of vector clocks does not allow such a-priori conclusions, and hence 

Armed with this insight, in this work we develop \emph{tree clocks}, a new data structure that replaces vector clocks in storing vector times.
In contrast to the flat structure of the traditional vector clocks, the dynamic hierarchical structure of tree clocks naturally captures ad-hoc communication patterns between processes.
In turn, this allows for join and copy operations that run in time that is roughly proportional to the number of entries that are being updated, and thus resulting in \emph{sublinear time}.
This leads to significant speedups in computing causal orderings in concurrent executions, as well as in performing further dynamic analyses once these causal orderings have been established.
As a data structure, tree clocks offer high versatility as they can be used in computing many different ordering relations.




==> extended-abstract/key_results.tex <==
\section{Key Results and Contributions}
\label{sec:key-contributions}

\begin{itemize}
  \item What are the most important \emph{one or two} empirical or theoretical
    results of this approach?
  \item What are the contributions that this paper makes to the state of the
    art? List them in an \texttt{itemize} section. Each contribution should be no more than a few sentences long.
  \item Clearly describe its advantages over past work, including how it overcomes their limitations.
\end{itemize}

\vspace{2cm}


Our contributions are as follows.
\begin{compactenum}
\item We introduce \emph{tree clock}, a new data structure for maintaining logical times in concurrent executions.
In contrast to the flat structure of the traditional vector clocks, the dynamic hierarchical structure of tree clocks naturally captures ad-hoc communication patterns between processes.
In turn, this allows for join and copy operations that run in \emph{sublinear time}.
As a data structure, tree clocks offer high versatility as they can be used in computing many different ordering relations.
\item We prove that tree clocks are an \emph{optimal data structure} for computing $\HB$, in the sense that, \emph{for every input trace}, the total computation time cannot be improved (asymptotically) by replacing tree clocks with any other data structure.
On the other hand, vector clocks do not enjoy this property.
%\item We prove that, for computing the $\HB$ partial order, tree clocks offer an optimality guarantee we call \emph{vector-time} (or \emph{vt-}) \emph{optimality}.
%Intuitively, vt-optimality guarantees that tree clocks are an \emph{optimal data structure} for $\HB$, in the sense that, \emph{for every input trace}, the total computation time cannot be improved (asymptotically) by replacing tree clocks with any other data structure.
%On the other hand, vector clocks do not enjoy this property.
\item We illustrate the versatility of tree clocks by presenting tree clock-based 
algorithms for the $\Maz$  and  $\SHB$ partial orders.
%\item \Andreas{Tree clocks for distributed?}
\item We perform a large-scale experimental evaluation of the tree clock data structure for computing the $\Maz$, $\SHB$ and $\HB$ partial orders, and compare its performance against the standard vector clock data structure.
Our results show that just by replacing vector clocks with tree clocks, the computation becomes between 1.73X and 2.53X faster on average.
Given our experimental results, we believe that replacing vector clocks by tree clocks in partial order-based algorithms can lead to significant improvements on many applications.

\end{compactenum}


==> extended-abstract/limitations.tex <==
\section{Limitations of the State of the Art}
\label{sec:limitations}

% \begin{itemize}
% \item What is the state of the art in this topic today (if any)?
% \item What are its limits?
% \end{itemize}

\begin{comment}
1. Timestamps are almost always implemented using vector datastructure - flat array style data structure
2. Fundamentally slow as updates need to be done by looking up the entire vector
3. In fact, this is Theta(k), and almost always a bottleneck
4. When special structure in the execution can be explouted, people do so to avoid the cost of full blown vector clocks
5. 
\end{comment}

State-of-the art techniques for analyzing concurrent programs by building partial orders often always rely on the use of \emph{vector clocks}.
Vector clocks are data-structures that encode \emph{timestamps} of events, and thus succinctly characterize the causal relationships between events in an execution of a concurrent program.
The timestamp of an event is \ucomment{here}.

==> extended-abstract/macros.tex <==
%!TEX root=main.tex

%\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
%\newtheorem{problem}{Problem}
%\newtheorem{proposition}{Proposition}
%\newtheorem{claim}{Claim}


\newtheorem{claim}{Claim}
\theoremstyle{plain}
\newtheorem{remark}{Remark}

\def\treeclocksexamplecaling{0.93}

\newcommand{\Paragraph}[1]{\noindent{\bf #1}}
\newcommand{\SubParagraph}[1]{\smallskip\noindent{\em #1}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

%%%% Math
\mathchardef\mhyphen="2D % Define a "math hyphen"
\newcommand{\Nats}{\mathbb{N}}
\newcommand{\Natsplus}{\Nats^{+}}
\newcommand{\Natsinf}{\mathbb{N}\cup\{\infty\}}
\newcommand{\Ints}{\mathbb{Z}}
\newcommand{\ov}{\overline}
\newcommand{\Index}{\mathsf{in}}
\newcommand{\wh}{\widehat}
\newcommand{\Width}{\mathsf{width}}
%\newcommand{\MWidth}{\mathsf{Mwidth}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\setpred}[2]{\{#1 \,|\, #2\}}

%%%% Concurrency notation
\newcommand{\tr}{\sigma}
\newcommand{\Trace}{\tr} %% Andreas
\newcommand{\lk}{\ell}
\newcommand{\Event}{e}
\newcommand{\ev}[1]{\langle #1\rangle}
\newcommand{\conf}{\asymp}
% \newcommand{\conf}{\Join} %% Andreas
\newcommand{\Confl}[2]{#1 \conf #2}
%\newcommand{\LConfl}[2]{#1 \amp #2}
\newcommand{\Vars}{\mathcal{V}}
\newcommand{\Algo}{\mathcal{A}}
\newcommand{\AlgoHB}{\mathcal{A}_{\operatorname{HB}}}


%% Ops
\newcommand{\opfont}[1]{\texttt{#1}}
\newcommand{\acq}{\opfont{acq}}
\newcommand{\rel}{\opfont{rel}}
\newcommand{\rd}{\opfont{r}}
\newcommand{\wt}{\opfont{w}}
\newcommand{\fork}{\opfont{fork}}
\newcommand{\join}{\opfont{join}}
\newcommand{\sync}{\opfont{sync}}
\newcommand{\acrl}{\opfont{acrl}}
\newcommand{\Read}{\rd}
\newcommand{\Write}{\wt}
\newcommand{\Acquire}{\acq}
\newcommand{\Release}{\rel}
\newcommand{\Sync}{\sync}
% \newcommand{\Read}{r} %% Andreas
% \newcommand{\Write}{w} %% Andreas
\newcommand{\LastWrite}{\operatorname{lw}}

\newcommand{\Concat}{\circ}
\newcommand{\ForkT}{\mathsf{fork}}
\newcommand{\SysReads}{\mathcal{R}}
\newcommand{\SysWrites}{\mathcal{W}}
\newcommand{\Project}{|}
\newcommand{\SymDiff}{\bigtriangleup}
\newcommand{\Domain}{\mathsf{dom}}
\newcommand{\Image}{\mathsf{img}}
\newcommand{\LocalTrace}{\kappa}
\newcommand{\True}{\operatorname{True}}
\newcommand{\False}{\operatorname{False}}
\newcommand{\Thread}{t}
\newcommand{\ThreadOf}[1]{\tid(#1)}
\newcommand{\Decor}{\operatorname{Decor}}
\newcommand{\Variable}{\operatorname{Variable}}
\newcommand*{\Match}[2][]{
\ifx\\#1\\%
  \mathsf{match}(#2)
\else
  \mathsf{match}_{#1}(#2)
\fi
}
%\newcommand*{\CS}[2][]{
%\ifx\\#1\\%
%  \mathsf{CS}(#2)
%\else
%  \mathsf{CS}_{#1}(#2)
%\fi
%}
%\newcommand*{\CCS}[2][]{
%\ifx\\#1\\%
%  \mathsf{CCS}(#2)
%\else
%  \mathsf{CCS}^{#1}(#2)
%\fi
%}
%\newcommand{\EarliestAcquire}[3]{\mathsf{EarliestAcquire}^{#1}_{#3}(#2)}
%\newcommand*{\CSL}[2][]{
%\ifx\\#1\\%
%  \mathsf{CSL}(#2)
%\else
%  \mathsf{CSL}^{#1}(#2)
%\fi
%}

%%%% Partial orders
\newcommand{\acr}[1]{\textsf{#1}}
\newcommand{\acrtr}{\operatorname{\acr{tr}}}
\newcommand{\TO}{\operatorname{\acr{TO}}}
\newcommand{\SHB}{\operatorname{\acr{SHB}}}
\newcommand{\Maz}{\operatorname{\acr{MAZ}}}
\newcommand{\FHB}{\operatorname{\acr{FHB}}}
\newcommand{\DC}{\operatorname{\acr{DC}}}
\newcommand{\HB}{\operatorname{\acr{HB}}}
\newcommand{\CP}{\operatorname{\acr{CP}}}
\newcommand{\WCP}{\operatorname{\acr{WCP}}}
\newcommand{\SDP}{\operatorname{\acr{SDP}}}
\newcommand{\WDP}{\operatorname{\acr{WDP}}}

\newcommand{\ord}[2]{\leq^{#1}_{\mathsf{#2}}}
\newcommand{\notord}[2]{\not\leq^{#1}_{\mathsf{#2}}}
\newcommand{\strictord}[2]{<^{#1}_{\mathsf{#2}}}
\newcommand{\unord}[2]{\parallel^{#1}_{\mathsf{#2}}}


\newcommand{\trord}[1]{\ord{#1}{\acrtr}}
\newcommand{\stricttrord}[1]{\strictord{#1}{\acrtr}}
\newcommand{\tho}[1]{\ord{#1}{\TO}}
\newcommand{\stricttho}[1]{\strictord{#1}{\TO}}
\newcommand{\nottho}[1]{\nototd{#1}{\TO}}
\newcommand{\hb}[1]{\ord{#1}{\HB}}
\newcommand{\unordhb}[1]{\unord{#1}{\HB}}
\newcommand{\stricthb}[1]{\strictord{#1}{\HB}}
\newcommand{\shb}[1]{\ord{#1}{\SHB}}
\newcommand{\maz}[1]{\ord{#1}{\Maz}}
\newcommand{\notshb}[1]{\notord{#1}{\SHB}}
\newcommand{\strictshb}[1]{\strictord{#1}{\SHB}}
% \newcommand{\cp}[1]{\ord{#1}{\CP}}
% \newcommand{\strictcp}[1]{\prec^{#1}_{\CP}}
% \newcommand{\notcp}[1]{\notord{#1}{\CP}}
% \newcommand{\wcp}[1]{\ord{#1}{\WCP}}
% \newcommand{\strictwcp}[1]{\prec^{#1}_{\WCP}}
% \newcommand{\notwcp}[1]{\notord{#1}{\WCP}} %{\not\leq^{#1}_{\mathsf{WCP}}}
\newcommand{\unordwcp}[1]{\unord{#1}{\WCP}}
% \newcommand{\sdp}[1]{\ord{#1}{\SDP}}
% \newcommand{\notsdp}[1]{\notord{#1}{\SDP}}%{\not\leq^{#1}_{\mathsf{SDP}}}

\newcommand{\Implies}{\Rightarrow}
% \newcommand{\Unordered}[3]{#1\parallel_{#2} #3}
\newcommand{\Ordered}[3]{#1 \not \parallel_{#2} #3}
\newcommand{\Refines}{\sqsubseteq}
\newcommand{\Acquires}{\operatorname{Acqs}}
\newcommand{\Releases}{\operatorname{Rels}}
\newcommand{\Reads}{\operatorname{Rds}}
\newcommand{\Writes}{\operatorname{Wts}}
\newcommand{\Threads}[1]{\operatorname{Thrds}_{#1}}
\newcommand{\Locks}[1]{\mathcal{L}_{#1}}
\newcommand{\Variables}[1]{\mathcal{V}_{#1}}
% \newcommand{\Locals}[1]{\mathcal{V}_{#1}}



\newcommand{\Path}{\rightsquigarrow}


\newcommand{\ReadsSet}{\mathsf{Rds}}
\newcommand{\WritesSet}{\mathsf{Wts}}

%% Tree Clocks notation
\newcommand{\LocalTime}[2]{\operatorname{lTime}^{#1}(#2)}
\newcommand{\VectorTime}{\operatorname{V}}
% \newcommand{\POTime}[3]{\VectorTime^{#1}_{#2}(#3)}
\newcommand{\POTime}[2]{C^{#1}_{#2}}
\newcommand{\VectorClock}{\operatorname{VC}}
\newcommand{\TreeClock}{\operatorname{TC}}
\newcommand{\CSmaller}{\sqsubseteq}
\newcommand{\CJoin}{\sqcup}
\newcommand{\CAssign}[2]{[#1\to +#2]}
\newcommand{\GTree}{\operatorname{T}}
\newcommand{\Root}{\operatorname{root}}
\newcommand{\ThreadMap}{\operatorname{ThrMap}}
\newcommand{\TNodes}{\mathcal{V}}
\newcommand{\TEdges}{\mathcal{E}}
\newcommand{\ChildrenQ}{\operatorname{Chld}}
\newcommand{\Left}{\operatorname{Left}}
\newcommand{\Right}{\operatorname{Right}}
\newcommand{\First}{\operatorname{First}}
\newcommand{\Parent}{\operatorname{Prnt}}
\newcommand{\Stack}{\mathcal{S}}
\newcommand{\Queue}{\mathcal{Q}}
\newcommand{\Worklist}{\mathcal{K}}
\newcommand{\Expanded}{}
\newcommand{\tid}{\operatorname{\mathsf{tid}}}
\newcommand{\clock}{\operatorname{clk}}
\newcommand{\pclock}{\operatorname{aclk}}
\newcommand{\VTime}[1]{\llbracket #1 \rrbracket}
\newcommand{\DataStructure}{\operatorname{DS}}
\newcommand{\VectorClockDataStructures}{\mathcal{C}}
\newcommand{\VTWork}{\operatorname{VTWork}}
\newcommand{\VCWork}{\operatorname{VCWork}}
\newcommand{\TCWork}{\operatorname{TCWork}}
\newcommand{\Time}{\mathcal{T}}
\newcommand{\vc}[1]{\langle{\texttt{#1}}\rangle}



%algorithm2e
\SetAlFnt{\small}
\SetInd{0.5em}{0.5em}

\SetKw{Break}{break}
\SetKwProg{MyFunction}{function}{}{}
\SetKwProg{MyRoutine}{routine}{}{}
\SetKwProg{MyProcedure}{procedure}{}{}
\SetKwFunction{FunctionCTInitialize}{{Init}}
\SetKwFunction{FunctionCTLessThan}{LessThan}
\SetKwFunction{FunctionCTJoin}{Join}
\SetKwFunction{FunctionVCJoin}{Join}
\SetKwFunction{FunctionCTSubRootJoin}{SubRootJoin}
\SetKwFunction{FunctionVCCopy}{Copy}
\SetKwFunction{FunctionCTMonotoneCopy}{MonotoneCopy}
\SetKwFunction{FunctionCTCopyCheckMonotone}{CopyCheckMonotone}
\SetKwFunction{FunctionCTVTime}{VectorTime}
\SetKwFunction{FunctionCTIncrement}{Increment}
\SetKwFunction{FunctionVCIncrement}{Increment}
\SetKwFunction{FunctionCTGet}{Get}
\SetKwFunction{RoutineTestDeque}{TestDeque}
\SetKwFunction{RoutineUpdatedNodesForJoin}{getUpdatedNodesJoin}
\SetKwFunction{RoutineUpdatedNodesForCopy}{getUpdatedNodesCopy}
\SetKwFunction{RoutineDetachNodes}{detachNodes}
\SetKwFunction{RoutineAttachNodesJoin}{attachNodesJoin}
\SetKwFunction{RoutineAttachNodesCopy}{attachNodesCopy}
\SetKwFunction{RoutineAttachNodes}{attachNodes}
\SetKwFunction{RoutinePushChild}{pushChild}
\SetKwFunction{RoutineInsertChild}{insertChild}
\SetKwFunction{ProcInitialize}{initialize}
\SetKwFunction{ProcAcquire}{acquire}
\SetKwFunction{ProcRelease}{release}
\SetKwFunction{ProcWrite}{write}
\SetKwFunction{ProcRead}{read}


\newcommand{\CTX}{\mathbb{X}}
\newcommand{\CTC}{\mathbb{C}}
\newcommand{\CTH}{\mathbb{H}}
\newcommand{\CTP}{\mathbb{P}}
\newcommand{\CTL}{\mathbb{L}}
\newcommand{\CTB}{\mathbb{B}}
\newcommand{\CTLW}{\mathbb{LW}}
\newcommand{\CTR}{\mathbb{R}}
\newcommand{\VCR}{\mathbb{R}}
\newcommand{\VCW}{\mathbb{W}}
\newcommand{\LWT}{\operatorname{LW}}
\newcommand{\EpochWrite}{\operatorname{EpochWrite}}
\newcommand{\EpochReads}{\operatorname{EpochReads}}
\newcommand{\LastReads}{\operatorname{LRDs}}
\newcommand{\AcquireQueue}{\operatorname{Acq}}
\newcommand{\ReleaseQueue}{\operatorname{Rel}}
\newcommand{\Enqueue}{\operatorname{Enqueue}}
\newcommand{\Dequeue}{\operatorname{Dequeue}}
\newcommand{\Front}{\operatorname{Front}}
\newcommand{\HeldLocks}{\operatorname{HeldLocks}}

\newcommand{\Andreas}[1]{\textcolor{blue}{\textbf{Andreas:}~#1}}
\newcommand{\FastHB}{\operatorname{FastHB}}
\newcommand{\Operation}{\operatorname{op}}
\newcommand{\NumEvents}{n}
\newcommand{\NumThreads}{k}
\newcommand{\NumVariables}{v}



%%%% Tools and Algorithms
\newcommand{\eraser}{\textsc{Eraser}\xspace}
\newcommand{\rapid}{\textsc{Rapid}\xspace}
\newcommand{\djitp}{\textsc{Djit}$^+$\xspace}
\newcommand{\fasttrack}{\textsc{FastTrack}\xspace}
\newcommand{\ZeroRevAlgo}{\textsf{SyncP}\xspace}
\newcommand{\tsan}{\textsc{ThreadSanitizer}\xspace}
\newcommand{\helgrind}{Helgrind\xspace}
\newcommand{\intelinspector}{Intel Inspector\xspace}
\newcommand{\ziptrack}{\textsc{ZipTrack}\xspace}
\newcommand{\roadrunner}{\textsc{RoadRunner}\xspace}
\newcommand{\rvpredict}{\textsf{RVPredict}\xspace}
\newcommand{\aerodrome}{\textsc{Aerodrome}\xspace}







\usetikzlibrary{arrows.meta,calc,decorations.markings,math,arrows.meta}


\preto\tabular{\setcounter{magicrownumbers}{0}}
\newcounter{magicrownumbers}




\setlength{\tabcolsep}{2.4pt}


\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)

\def \darkred {black!20!red}
\def \darkgreen {black!40!green}
\SetKw{Continue}{continue}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{gray}{#1}}
\SetCommentSty{mycommfont}

\newlist{compactenum}{enumerate}{3} % 3 is max-depth
\setlist[compactenum]{label=\arabic*., nosep,leftmargin=*}
\crefname{compactenumi}{Item}{Items}

\makeatletter
\newcommand*{\centerfloat}{%
  \parindent \z@
  \leftskip \z@ \@plus 1fil \@minus \textwidth
  \rightskip\leftskip
  \parfillskip \z@skip}
\makeatother

\newcommand{\ucomment}[1]{\textcolor{red}{#1}}

%\input{exec_macros}


==> extended-abstract/main_artifacts.tex <==
\section{Main Artifacts}
\label{sec:main-artifacts}

\begin{itemize}
\item What are the key artifacts presented in your paper: a
  methodology, a hardware design, a software algorithm, an
  optimization or control technique, etc.?
  \item How were your artifacts implemented and evaluated? 
\end{itemize}


\vspace{2cm}



==> extended-abstract/motivation.tex <==
\section{Motivation}
\label{sec:motivation}

\begin{comment}
1. analysis of concurrent programs is important - model checking, bug finding. 
2. To reduce the effectiveness of each of these techniques, partial orders are used -- reduce state space (which might be exponentially otherwise)
3. Timestamps are used to encode the causal relationships induced by the partial order
4. What is timestamp
5. Since timestamp computation happens frequently, it can be the bottleneck
6. Thus it is important to speedup cost of computation of timestamps
\end{comment}

The analysis of multi-threaded programs is one of the major challenges in building reliable and scalable software systems.
The large space of communication interleavings in such programs poses a significant challenge to the programmer, as intended invariants can be broken by unexpected communication patterns.
Consequently, significant efforts are made towards understanding and detecting concurrency bugs efficiently
\cite{lpsz08,Shi10,Tu2019,SoftwareErrors2009,boehmbenign2011,Farchi03}.


\begin{itemize}
\item What is the problem your work attacks? Be specific.
\item Why is it an important problem?
\end{itemize}

\vspace{1em}

\noindent
Articulate the importance of this problem to the broader ASPLOS
community, using as little jargon as possible. \emph{Be specific}
about the problem you are addressing; it should be the one that your
paper directly addresses.


==> extended-abstract/packages.tex <==
\usepackage[utf8]{inputenc} 
\usepackage{amsmath, amsthm, amsfonts}
\usepackage{thmtools}
\usepackage[english]{babel}
\usepackage{pdfpages}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{caption}
\usepackage{longtable}
\usepackage{booktabs}
\usepackage{tabu}
\usepackage[referable]{threeparttablex}
\usepackage{varwidth}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{wrapfig}
\usepackage{lipsum}
\usepackage{stmaryrd}
\usepackage{float}

\usepackage{pifont}

\usepackage[ruled, linesnumbered,noend]{algorithm2e}

\usepackage{parskip}

\usepackage{hyperref}
\usepackage{thm-restate}
\usepackage[capitalise]{cleveref}

\crefname{figure}{Figure}{Figure}
\crefformat{footnote}{#2\footnotemark[#1]#3}
\usepackage{tikz}
\usepackage{tikz-qtree}
%\usepackage{kerkis}
\usepackage{comment}
%%\usepackage{xfrac}

% \usepackage{todonotes}
\usepackage{tikz}
\usetikzlibrary{fit,arrows,automata,shapes,decorations,decorations.markings,calc, matrix,decorations.pathmorphing, patterns,backgrounds}

\usepackage{bm}
\usepackage{pgfplots}
\usepackage{enumitem}



\usepackage{pbox}

\usepackage{appendix}
\usepackage{calc}
\usepackage{fp}
\usepackage{multirow}
\usepackage{pbox}

\usepackage{etoolbox}

\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}

\usepackage{arydshln}





==> extended-abstract/why_asplos.tex <==
\section{Why ASPLOS}
\label{sec:why-asplos}



% ASPLOS emphasizes multidisciplinary research; explain how this
%   paper emphasizes synergy of \emph{two or more ASPLOS areas}: architecture,
%   programming languages, operating systems, and related areas (broadly
%   interpreted).
  
  
%   \vspace{2cm}

Concurrency is one of the most studied topics today among different communities (systems, architecture, PL), be it multithreading or distributed systems.
The community of ASPLOS, in particular, has a long tradition in analyzing and optimizing parallel programs, and offering parallel support for programming languages tasks.
Our work lies in the intersection of parallelism, programming languages and algorithms, and delivers improvements in both theory and practice of the analysis of concurrent programs, and hence has a very tight fit to the ASPLOS research.
Moreover, as our key contribution is a new versatile data structure (as opposed to a dedicated framework), we anticipate that tree clocks will be quickly picked up by the ASPLOS community and find applications beyond the ones presented in this work.
Our "Related Work" section of the paper suggests some immediate next steps in this direction.


\textcolor{red}{
\begin{itemize}
\item Concurrency is an important problem studied by  Same for race detection.
\item Systems/OS - concurrency bugs are, till this date, common occurences leading to system failure
\item Architecture - hardware level multi-threading and hardware level detection
\item PL - researchers have previously argued for the development of an "always-on" race detectors so as to allow for "race exceptions" [cite Qadeer and Tesiran, Goldilocks: A Race and
Transaction-Aware Java Runtime] [cite Conflict exceptions: simplifying concurrent language semantics with precise hardware exceptions for data-races]
\item Our work fundamentally changes the way algorithms for race detection and other analysis for inferring concurrency relationships between events (perhaps consensus algorithms) are implemented.
\end{itemize}
}






==> fasthb.tex <==
\section{$\FastHB$}\label{sec:fasthb}


\Paragraph{Happens-before ($\HB$).}








\Paragraph{Last reads.}
Given a trace $\Trace$ and a write event $\Write$ on a variable $x$, we define the \emph{last reads} of $\Write$ 
as the read events on $x$ that appear between $\Write$ and the last appearance of a write event $\Write'$ on $x$ that precedes $\Write$ in $\Trace$.
Formally,
\begin{align*}
\LastReads^{\Trace}(\Write)=\{&\Read\in \Reads{\Trace}\colon \Variable(\Read)=x \text{ and }\\
& \not\exists \Write' \text{ s.t. }
\Variable(\Write)=x \text{ and } \Read<^{\Trace}\Write'<^{\Trace}\Write \}\ .
\end{align*}
Our motivation behind this definition comes from the following lemma.

\smallskip
\begin{restatable}{lemma}{lemforgetreads}\label{lem:forget_reads}
Consider any trace $\Trace$, variable $x$ and write event $\Write$ on $x$.
If $\Write$ is the first racy write event of $\Trace$ on $x$, then one of the following holds.
\begin{compactenum}
\item $\Trace$ has a data race $(\Write', \Write)$.
\item There exists a read event $\Read\in \LastReads^{\Trace}(\Write)$ such that $(\Read, \Write)$ is a data race of $\Trace$.
\end{compactenum}
\end{restatable}


\Andreas{With epochs on both writes and reads, every read and write event is tested at most once.}


\input{algorithms/algo_fasthb}


\smallskip
\begin{restatable}{theorem}{thmfasthb}\label{thm:fasthb}
$\FastHB$ is a vector-time optimal race detector.
\ucomment{I deleted the def. of Variables in the prelim.}
Moreover, on input trace $\Trace$, for every variable $x\in \Variables{\Trace}$,
$\FastHB$ reports at least the first $\HB$ warning event $\Write(x)$ and $\Read(x)$
\end{restatable}


==> figures/fig_hb_race.tex <==
\begin{figure}
\execution{3}{
\figev{1}{$\Acquire(\textcolor{blue}{\ell_1})$}
\figev{1}{$\mathbf{\Write(x)}$}
\figev{1}{$\Release(\textcolor{blue}{\ell_1})$}
\figev{2}{$\Acquire(\textcolor{blue}{\ell_1})$}
\figev{2}{$\Read(x)$}
\figev{2}{$\Release(\textcolor{blue}{\ell_1})$}
\figev{3}{$\mathbf{\Read(x)}$}
\orderedgewithlabel{1}{3}{0.5}{2}{4}{-0.5}{\small $\HB$}{above}
}
\caption{
An $\HB$ race $(\Event_{2}, \Event_{7})$ implies the existence of a data race, 
by delaying the execution of $\Event_{2}$ until $\Event_{7}$.
}
\label{fig:hb_race}
\end{figure}

==> figures/fig_hb_suboptimal.tex <==
\begin{figure}
\executionVar{5}{3}{
\figev{1}{$\Acquire(\textcolor{blue}{\ell_1})$}
\figev{1}{$\Release(\textcolor{blue}{\ell_1})$}
\figev{2}{$\Acquire(\textcolor{blue}{\ell_1})$}
\figev{2}{$\Release(\textcolor{blue}{\ell_1})$}
\figev{3}{$\dots$}
\figev{4}{$\Acquire(\textcolor{blue}{\ell_1})$}
\figev{4}{$\Release(\textcolor{blue}{\ell_1})$}
\figev{5}{$\Acquire(\textcolor{blue}{\ell_1})$}
\figev{5}{$\Release(\textcolor{blue}{\ell_1})$}
\figev{4}{$\Acquire(\textcolor{blue}{\ell_1})$}
\figev{4}{$\Release(\textcolor{blue}{\ell_1})$}
\figev{5}{$\Acquire(\textcolor{blue}{\ell_1})$}
\figev{5}{$\Release(\textcolor{blue}{\ell_1})$}
\figev{4}{$\dots$}
\figevStale{5}{$\dots$}
}
\caption{
Every event after $\Event_{10}$ leads to a vector clock operation that modifies a single entry of the corresponding vector clock, but takes $O(\NumThreads)$ time.
}
\label{fig:hb_suboptimal}
\end{figure}


==> figures/fig_intuition2.tex <==
\begin{figure}
\execution{4}{
\figev{1}{$\Acquire(\textcolor{blue}{\ell_1})$}
\figev{1}{$\Release(\textcolor{blue}{\ell_1})$}
\figev{3}{$\Acquire(\textcolor{blue}{\ell_1})$}
\figev{3}{$\Release(\textcolor{blue}{\ell_1})$}
\figev{2}{$\Acquire(\textcolor{\darkred}{\ell_2})$}
\figev{2}{$\Release(\textcolor{\darkred}{\ell_2})$}
\figev{3}{$\Acquire(\textcolor{\darkred}{\ell_2})$}
\figev{3}{$\Release(\textcolor{\darkred}{\ell_2})$}
\figev{4}{$\Acquire(\textcolor{\darkred}{\ell_2})$}
\figev{4}{$\Release(\textcolor{\darkred}{\ell_2})$}
\figev{3}{$\Acquire(\textcolor{\darkgreen}{\ell_3})$}
\figev{3}{$\Release(\textcolor{\darkgreen}{\ell_3})$}
\figev{4}{$\Acquire(\textcolor{\darkgreen}{\ell_3})$}
\figev{4}{$\Release(\textcolor{\darkgreen}{\ell_3})$}
\orderedgewithlabel{1}{2}{0.5}{3}{3}{-0.5}{\small $\HB$}{above}
\orderedgewithlabel{2}{6}{0.5}{3}{7}{-0.5}{\small $\HB$}{above}
\orderedgewithlabel{3}{8}{0.5}{4}{9}{-0.5}{\small $\HB$}{above}
\orderdashededgewithlabel{3}{12}{0.5}{4}{13}{-0.5}{\small $\HB$}{above}
}
\caption{
Illustration of the second insight behind tree clocks.
}
\label{fig:intuition2}
\end{figure}

==> intuition-old.tex <==
%!TEX root=main.tex

\subsection{Intuition}\label{subsec:intuition}



Similar to vector clocks, a tree clock is a data structure for storing vector times.
In contrast to the flat structure of a vector clock, a tree clock stores time information hierarchically in a tree structure. %, with some additional annotations.
Each node of the tree represents the clock of a thread, 
while the tree structure represents clock information 
that has been obtained transitively via intermediate threads.
Below we illustrate two principles behind tree clocks in full generality.
For conciseness, we use the operation $\Sync(\lk)$ to 
denote the effect of two events by the same thread in succession, performing 
the operation sequence $\Acquire(\lk) \Release(\lk)$.


\Paragraph{1.~Direct monotonicity.}
Our first insight is a form of direct monotonicity.
Let us say we are computing the $\HB$ order for the
trace $\Trace$ of \cref{subfig:intuition1}, and assume that
we are currently processing the 
acquire event in $\Event_{7}$.
At this point, an $\HB$ ordering is discovered $\Event_{6} \stricthb{\Trace} \Event_{7}$ (dashed), 
and thread $\Thread_4$ (performing event $e_7$)
transitively \emph{learns} about all events known to 
thread $\Thread_3$ by performing a join operation (`$\CTC_{\Thread_4}.\FunctionVCJoin(\CTC_{\lk})$').
A careful look at what happens in the algorithm prior to this reveals the following.
\begin{compactenum}
\item Thread $\Thread_3$ has learned of event $\Event_1$ of $\Thread_1$ transitively, by having learned of event $\Event_2$ of thread $\Thread_2$.
\item Thread $\Thread_4$ has learned of event $\Event_4$ of thread $\Thread_2$.
\end{compactenum}
Thus we have a form of \emph{direct monotonicity}:~since $\Thread_4$ already knows of a later event of $\Thread_2$ than $\Thread_3$, any events that are known to $\Thread_3$ via $\Thread_2$, they are also known to $\Thread_4$.
Hence, we don't need to iterate over the corresponding threads (thread $\Thread_1$ in this case), as the $\max$ operation of the join will be vacuous.







%\input{figures/fig_intuition2}
\Paragraph{2.~Indirect monotonicity.}
Our second insight is a form of indirect monotonicity.
Consider the trace $\Trace$ of \cref{subfig:intuition2}, and assume that the algorithm is currently processing the lock-acquire event $\Event_{7}$ (dashed edge).
At this point, an $\HB$ ordering is discovered $\Event_{6}<^{\Trace}_{\HB}\Event_{7}$ (dashed), and thus thread $\Thread_4$ learns transitively of all events known to thread $\Thread_3$ by performing a join operation.
Since thread $\Thread_4$ does not yet know of $\Event_{6}$, there is no directed monotonicity exploited here, and we will proceed to examine all other threads known to thread $3$.
Note, however, the following.
\begin{compactenum}
\item Thread $\Thread_3$ has learned of event $\Event_3$ of thread $\Thread_2$ through its own event $\Event_4$.
Similarly, it has learned of event $\Event_1$ of thread $\Thread_1$  through its own event $\Event_2$.
\item Thread $\Thread_4$ has learned of event $\Event_4$ of thread $\Thread_3$.
\end{compactenum}
Thus we have a form of \emph{indirect monotonicity}:~since $\Thread_4$ knows of $\Event_4$ of $\Thread_3$, any events that are known to $\Thread_3$ \emph{via earlier events}, they are also known to $\Thread_4$.
Thus, we don't need to iterate over the corresponding threads (thread $\Thread_1$ in this case), as the $\max$ operation of the join will be vacuous.





Direct and indirect monotonicity reason about transitive orderings.
The flat structure of vector clocks misses the transitivity of information sharing, and thus arguments based on monotonicity are lost, resulting in vacuous operations during vector clock joins.
On the other hand, tree clocks maintain transitivity in their hierarchical structure.
In turn, this allows to reason about direct and indirect monotonicity, and thus often avoid redundant operations.

==> optimality.tex <==
\subsection{Work Optimality of tree clocks}\label{subsec:vtoptimality}

Finally, in this section we prove the optimality of tree clocks for race detection,
in the sense that replacing tree clocks with any other data structure cannot reduce
the asymptotic running time of the algorithm.







==> race_prediction.tex <==
%\section{Tree Clocks in Race Prediction}\label{sec:race_prediction}
%
%In the previous section we saw how tree clocks can be used for computing the happens-before partial order.
%However, as a data structure, tree clocks  are not tied to this domain, but can be broadly used (either directly or with small modifications) in other settings of dynamic analyses.
%In this section we show how tree clocks can replace vector clocks in computing other partial orders that are used in state-of-the-art data-race predictors.
%In particular, we target the following partial orders.
%
%\begin{compactenum}
%\item Schedulably-Happens-Before ($\SHB$)~\cite{Mathur18}.
%\item Weak-Causally-Precedes ($\WCP$)~\cite{Kini17}.
%\item Doesn't-commute ($\DC$)~\cite{Roemer18}.
%\item Strong-Dependently-Precedes ($\SDP$)~\cite{Genc19}.
%\end{compactenum}
%
%Due to space restrictions, we only develop $\SHB$ and $\WCP$ in detail, 
%while we refer to \cref{sec:app_race_predictors} for $\DC$ and $\SDP$.



%\input{wcp}


==> tables/counters.tex <==
\begin{table*}
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{1.2}
\small
\centering
\begin{tabular}{|c|c|c|c||c|c|c|}
\hline
\textbf{ Benchmark} &\multicolumn{3}{c||}{ {\textsf{HB}}} & \multicolumn{3}{c|}{ {\textsf{SHB}}}\\
\hline
&{ \textbf{VT-Work}} & { \textbf{TC-Work}} & { \textbf{VC-Work}} &{ \textbf{VT-Work}} & { \textbf{TC-Work}} & { \textbf{VC-Work}}\\
\hline
\hline
jigsaw & 6.9K & 17K & 130K & 2.0M & 5.0M & 37M\\
allocvector & 7.4K & 10K & 308K & 1.1M & 1.1M & 3.0M\\
startup & 6.5K & 16K & 58K & 3.9M & 32M & 143M\\
ftpserver & 12K & 23K & 131K & 104K & 149K & 594K\\
batik & 54K & 157K & 734K & 101M & 253M & 1.1B\\
xml & 19K & 31K & 592K & 34M & 65M & 1.4B\\
derby & 35K & 91K & 281K & 1.8M & 3.0M & 6.9M\\
biojava & 8.0K & 23K & 62K & 28M & 249M & 884M\\
elevator & 47K & 98K & 271K & 53K & 270K & 1.3M\\
luindex & 207K & 622K & 1.2M & 95M & 489M & 1.2B\\
lusearch & 167K & 501K & 2.7M & 109M & 321M & 1.7B\\
cryptorsa & 422K & 836K & 3.1M & 44M & 101M & 526M\\
bbuffer & 243K & 368K & 1.4M & 483K & 1.1M & 8.1M\\
zxing & 166K & 436K & 4.0M & 742M & 1.2B & 8.2B\\
chinserts & 912K & 2.0M & 4.0M & 48M & 66M & 96M\\
sor & 1.7M & 3.6M & 6.3M & 405M & 1.0B & 3.0B\\
chadddelete & 711K & 1.6M & 14M & 72M & 78M & 183M\\
hsqldb & 233K & 656K & 18M & 46M & 64M & 829M\\
eclipse & 804K & 2.2M & 21M & 211M & 290M & 1.4B\\
derby & 1.1M & 3.2M & 6.2M & 230M & 591M & 1.1B\\
tomcat & 1.8M & 2.9M & 36M & 384M & 440M & 2.4B\\
tradesoap & 535K & 791K & 54M & 679M & 715M & 8.6B\\
xalan & 1.4M & 3.6M & 14M & 68M & 187M & 857M\\
bufwriter & 1.2M & 3.5M & 16M & 3.5M & 15M & 82M\\
tradebeans & 574K & 830K & 54M & 679M & 715M & 8.7B\\
chiterator & 3.0M & 7.2M & 52M & 62M & 74M & 227M\\
crypto & 5.9M & 10.0M & 155M & 424M & 660M & 10B\\
cassandra & 30M & 68M & 4.4B & 1.9B & 2.1B & 44B\\
raxextended & 94M & 251M & 3.9B & 180M & 490M & 7.9B\\
\hline
\end{tabular}
\caption{
Comparison of the total work performed by the vector clock and tree clock algorithms.
}
\label{tab:counters}
\end{table*}

==> tables/tab_times.tex <==
%!TEX root=../main.tex

\begin{table}
\caption{
Running times for$\HB$ and $\SHB$ using vector clocks (\textsf{VC}) and tree clocks (\textsf{TC}).
The geometric means of the speedups are $\operatorname{GMean}_{\HB}=2$ and $\operatorname{GMean}_{\SHB}=1.75$.
}
\label{tab:times}
\setlength\tabcolsep{2.5pt}
\renewcommand{\arraystretch}{1.2}
\small
\centerline{
\begin{tabular}{|c|c|c|c|||c|c||c|c|}
\hline
\textbf{ Benchmark} & { $\NumEvents$} & { $\NumThreads$} & { $\NumVariables$} &\multicolumn{2}{c||}{ {\textsf{HB}}} & \multicolumn{2}{c|}{ {\textsf{SHB}}}\\
\hline
&&&&{ \textbf{VC}} & { \textbf{TC}} & { \textbf{VC}} & { \textbf{TC}}\\
\hline
\hline
jigsaw & 3.1M & 12 & 103K & 0.06s & 0.07s & 1.09s & 0.73s \\
allocvector & 29K & 103 & 10K & 0.07s & 0.03s & 0.29s & 0.25s \\
startup & 31M & 5 & 307K & 0.07s & 0.05s & 5.39s & 2.34s \\
ftpserver & 49K & 12 & 5.5K & 0.08s & 0.05s & 0.10s & 0.12s \\
batik & 157M & 7 & 4.9M & 0.09s & 0.09s & 42.73s & 32.85s \\
xml & 42M & 43 & 1.9M & 0.09s & 0.10s & 16.25s & 4.34s \\
derby & 1.4M & 5 & 185K & 0.10s & 0.11s & 0.51s & 0.67s \\
biojava & 221M & 4 & 121K & 0.12s & 0.08s & 40.23s & 22.15s \\
elevator & 211K & 6 & 725 & 0.14s & 0.09s & 0.18s & 0.21s \\
luindex & 397M & 3 & 2.5M & 0.18s & 0.15s & 1m8s & 49.36s \\
lusearch & 217M & 8 & 5.2M & 0.19s & 0.16s & 51.69s & 28.46s \\
cryptorsa & 58M & 9 & 1.7M & 0.19s & 0.15s & 18.21s & 6.68s \\
bbuffer & 504K & 16 & 34 & 0.21s & 0.07s & 0.37s & 0.25s \\
zxing & 546M & 15 & 37M & 0.21s & 0.11s & 4m33s & 2m33s \\
chinserts & 24M & 4 & 5.8M & 0.29s & 0.12s & 9.84s & 11.22s \\
sor & 606M & 5 & 1.0M & 0.31s & 0.23s & 2m47s & 2m44s \\
chadddelete & 8.0M & 23 & 2.6M & 0.31s & 0.19s & 3.76s & 10.51s \\
hsqldb & 18M & 44 & 945K & 0.34s & 0.13s & 9.76s & 3.92s \\
eclipse & 90M & 15 & 10M & 0.46s & 0.27s & 31.23s & 20.27s \\
derby & 471M & 3 & 20M & 0.52s & 0.39s & 1m27s & 1m10s \\
tomcat & 49M & 48 & 6.1M & 0.59s & 0.31s & 36.57s & 20.56s \\
tradesoap & 39M & 221 & 2.8M & 0.61s & 0.15s & 1m22s & 13.79s \\
xalan & 122M & 7 & 4.4M & 0.64s & 0.39s & 32.56s & 21.62s \\
bufwriter & 11M & 7 & 56 & 0.74s & 0.20s & 2.18s & 0.90s \\
tradebeans & 39M & 222 & 2.8M & 0.93s & 0.14s & 1m20s & 19.20s \\
chiterator & 14M & 16 & 3.0M & 0.95s & 0.34s & 5.50s & 4.08s \\
crypto & 294M & 43 & 13M & 2.30s & 0.63s & 2m24s & 41.75s \\
cassandra & 259M & 173 & 9.9M & 37.43s & 2.95s & 7m41s & 53.30s \\
raxextended & 304M & 26 & 48 & 49.94s & 10.10s & 1m11s & 21.76s \\
\hline
\textbf{Totals} & - & - & - & \textbf{1m38s} & \textbf{17.84s} & \textbf{29m7s} & \textbf{13m0s} \\
\hline
\end{tabular}
}
\end{table}


==> vector_clocks.tex <==
\subsection{The Vector Time Interface}\label{subsec:vector_clocks}



\Paragraph{The vector-clock interface.}
We say that a data structure $\DataStructure$ \emph{implements the vector-clock-interface} (or \emph{vc-interface}) if it represents a vector-time, denoted by $\VTime{\DataStructure}$, and supports updates of its state with vector-time operations.

\Paragraph{Vector-clock work.}
Consider a streaming algorithm $A$ and let $\VectorClockDataStructures=\{ C_1, \dots, C_m \}$ be the set of data structures maintained by $A$ that implement the vector interface.
Consider that $A$ is executed on some input trace $\Trace$.
Given some $i\in[m]$ and some integer $j\in [|\Trace|]$, we denote by $C_i^j$ the state of the data structure $C_i$ after $A$ has processed the $j$-th event of $\Trace$.
The  \emph{vector-clock-work} (or \emph{vc-work}) of $A$ on $\Trace$ is defined as

\begin{align*}
\VTWork_{A}(\Trace) = \sum_{i\leq m} \sum_{j\leq |\Trace|} \left|\left\{\Thread\colon \VTime{C_i^{j}}(\Thread) \neq \VTime{C_i^{j-1}}(\Thread) \right\}\right|\ .
\end{align*}


In words, each term in the sum counts the number of entries of $C_i$  that are updated by $A$ as the algorithm processes the next event of the input.
Overall, $\VTWork_{A}(\Trace)$ counts the total number of vector-clock updates made by $A$ as it processes the whole of $\Trace$.


\Paragraph{Vector-clock optimality.}
The goal of a vc data structure $\DataStructure$ is to provide the vc-interface to $A$ as efficiently as possible.
Let $\Time_{A}(\Trace)$ be the total time spent by $A$ for vector-clock operations.
We say that $\DataStructure$ is \emph{vector-clock-work optimal} (or \emph{vc-work optimal}) for $A$ if
\begin{align*}
\Time_{A}(\Trace) = O(\VTWork_{A}(\Trace))\ .
\end{align*}
In words, the amount of time that $\DataStructure$ instances spend in vc operations is proportional to the total number of updates to their state by $A$ (i.e., the total amount of vc-work by $A$).


==> wcp.tex <==
%!TEX root=main.tex

\subsection{Weak-Causally-Precedes}\label{subsec:wcp}


\Paragraph{The $\WCP$ partial order.}
Weak-causally-precedes is a partial order introduced in~\cite{Kini17}.
It is a sound weakening of $\HB$ and hence can report more races.
Intuitively, this is achieved by not always ordering critical sections on the same lock.
To maintain soundness, $\WCP$ is closed under left and right composition with $\HB$.

\Paragraph{$\WCP$ with tree clocks.}
\cref{algo:wcp} shows $\WCP$ using tree clocks.
There are two important observations  for replacing vector clocks in $\WCP$ with tree clocks.
First, the copies in \cref{line:wcp_copyread,line:wcp_copywrite}, occurring when the algorithm processes a lock-release event $\Release$ are indeed monotone.
This monotonicity holds due to the corresponding joins in \cref{line:wcp_readjoin} and \cref{line:wcp_writejoin} 
that occur while the algorithm processes the critical section of $\Release$.

Second, $\WCP$ does not contain the thread order $\TO$, i.e., there might exist events $\Event_1, \Event_2$ such that
$\Event_1 \stricttho{\Trace} \Event_2$ but $\Event_1 \unordwcp{\Trace} \Event_2$.
Due to this, when we perform a join operation from a tree clock $\CTX$ to a tree clock $\CTC_{\Thread}$ (where $\CTC_{\Thread}$ holds the $\WCP$ time of the current event of thread $\Thread$), monotonicity does not generally hold:
it could be that the clock of some thread $\Thread'$ has progressed in $\CTC_{\Thread}$ compared to $\CTX$, but $\CTC_{\Thread}$ is not aware of the events that hang in the subtree of $\CTX$ rooted the a node $u$ with $u.\tid=\Thread'$.
However, a closer observation reveals that, because $\WCP$ is closed under composition with $\HB$,
this can only happen when $\Thread'=\Thread$, and thus $u$ is the root of $\CTC_{\Thread}$.
Hence, monotonicity only fails for nodes in the first level of $\CTC_{\Thread}$, while it holds for all other nodes.
We accommodate this corner case by modifying the general $\FunctionCTJoin$ function to $\FunctionCTSubRootJoin$
--- the latter is identical to the former with the following small modifications.
\begin{compactenum}
\item The if block in \cref{line:functionctjoinifroot} is not executed.
\item The if block in \cref{line:routineupdatednodesforjoinifbreak} is not executed if $u'.\tid=\Thread$.
\item The body of the while loop in \cref{line:routineattachnodesmainloop} is skipped $u'.\tid=\Thread$.
\end{compactenum}

$\FunctionCTSubRootJoin$ is called in \cref{line:wcp_readsubjoin} and \cref{line:wcp_writesubjoin1}  of \cref{algo:wcp}.



\input{algorithms/algo_wcp}
